Rao-Blackwellized Stochastic Gradients for Discrete Distributions

We wish to compute the gradient of an expectation over a finite or countably infinite sample space having $K \leq \infty$ categories. When $K$ is indeed infinite, or finite but very large, the relevant summation is intractable. Accordingly, various stochastic gradient estimators have been proposed. In this paper, we describe a technique that can be applied to reduce the variance of any such estimator, without changing its bias---in particular, unbiasedness is retained. We show that our technique is an instance of Rao-Blackwellization, and we demonstrate the improvement it yields on a semi-supervised classification problem and a pixel attention task.

==> 5c_astro_results.tex <==
Locating and characterizing galaxies in telescope images is an import problem in astronomy.
The deep generative model for galaxy images proposed in~\cite{regier2015deep} achieves state-of-the-art results,
but only for images cropped to have a single galaxy at their center.
In this section, we use a hard-attention mechanism~\cite{mnihattnmechanism, GregorDRAW} to remove the restriction that galaxies must be centered in images.

Our generative model is as follows.
For each image, we sample a particular two-vector representing the pixel at the imaged galaxy's center:
\begin{align}
    z \sim \mathrm{Categorical}(H \times W).
\end{align}
Here $H$ and $W$ are respectively the height and width, in pixels, of the images.
Next, as in~\cite{regier2015deep}, to represent the shape and brightness of the galaxy, we sample an eight-dimensional vector:
\begin{align}
    y \sim \mathcal{N}(0, I).
\end{align}
Finally, for each pixel $(h, w) \in H \times W$, the pixel intensity is
\begin{multline}
    x_{h,w} | y, z \sim \\
     \mathcal{N}( \mu(y)[h - z_0, w - z_1],  \Sigma(y)[h - z_0, w - z_1] ).
\end{multline}
Here $\mu$ and $\Sigma$ are neural networks that return a grid of, respectively, means and variances.

In this way, $x \in \mathbb{R}^{H \times W}$ is a random sample of an image containing a single non-centered galaxy.

Hence, not only do we need to learn the generative model for a single galaxy, but we need to infer the pixel at which the galaxy is centered. Our two latent variables are $z_n$ and $y_n$. We find a variational approximation to the posterior using an approximating family of the form 
\begin{align}
    z_n | x_n \sim \mathrm{Categorical}(\zeta(x_n))
\end{align}
and
\begin{align}
    y_n | x_n, z_n \sim \mathcal{N}(h_\mu(x_n, z_n), h_\Sigma(x_n, z_n)),
\end{align}
where $\zeta$, $h_\mu$, and $h_\Sigma$ are neural networks. See appendix for architecture details. 


We minimize 
\begin{align}
\text{KL}(q(y_n, z_n|x_n) \| p(y_n, z_n | x_n)),
\end{align}
which is equivalent to maximizing the ELBO
\begin{align}
    \E_{z_n \sim q(z_n)} &\Big[\E_{y_n \sim q(y_n|z_n)}\Big[\log p(x_n | y_n, z_n) \notag \\
    & + \log p(z_n) + \log(y_n) + \notag \\
    & - \log q(z_n | x_n) - \log q(y_n | z_n, x_n) \Big]\Big].
\end{align}
Since $y_n$ is a continuous random variable, we use the reparameterization trick for the inner expectation. We use the REINFORCE+CV estimator to compute the discrete expectation over $z_n$. In this case, there are $H \times W$ categories for $z_n$, so procedures whose computational cost scales linearly with the number of categories would likely be intractable. 

We again examine the gains of Rao-Blackwellizing the REINFORCE+CV gradient estimator.
The negative ELBO per epoch is shown in Figure~\ref{fig:galaxy_optimization_paths}. We simulate new galaxy images at each epoch: an epoch consists of 200 batches, each batch having 64 images. Rao-Blackwellizing improves the convergence rate of the optimization. 

Figure~\ref{fig:galaxy_rb_reinforce_compare} compares Rao-Blackwellization to na\"{i}ve minibatching. It shows the loss per epoch of summing out $k = 3$ categories, thus evaluating the objective function four times, compared to averaging four independent samples of the REINFORCE+CV gradient estimate. Here too, Rao-Blackwellization provides an improvement. 

\begin{figure}[tb]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{./results/galaxy_trace_plots.png}
    \end{subfigure}
    \caption{Negative ELBO per iteration for REINFORCE+CV, Rao-Blackwellized by summing $k = 0, 1$, or 3 components, for the galaxy attention experiment.  }
    \label{fig:galaxy_optimization_paths}
\end{figure}

\begin{figure}[tb]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{./results/galaxy_comparison_plot.png}
    \end{subfigure}
    \caption{We compare summing $K = 3$ categories for Rao-Blackwellization, against sampling four times for REINFORCE+CV, in the galaxy attention experiment. }
    \label{fig:galaxy_rb_reinforce_compare}
\end{figure}
% e]{In the caption, ``summing out'' is hard to understand. Maybe say $k$? Or $k$ categories summed?}

Finally, we show the original image against the reconstructed image in Figure~\ref{fig:galaxy_reconstructions}. Note that we simulated images of size $31\times 31$ pixels, for a total of 961 discrete categories. The experiment shows that summing out a few high-probability categories can lead to material speed-ups in the optimization, and Figure~\ref{fig:galaxy_reconstructions} shows that the optimization is ultimately successful.

\begin{figure}[tb]
    \centering
    \vspace{-0.15in}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{./results/galaxy_figs.png}
    \end{subfigure}
    \caption{(Left) The original simulated galaxy image. (Right) The reconstructed galaxy images. }
    \label{fig:galaxy_reconstructions}
        \vspace{-0.15in}
\end{figure}


==> introduction_old.tex <==
\section{Introduction}\label{sec:introduction}
Let $z$ be a discrete random variable over $K \leq \infty$ categories, with distribution $q_\eta(z)$ parametrized by a real vector $\eta$ and differentiable in $\eta$. We aim to minimize 
\begin{align}
\mathcal L(\eta) := \mathbb E_{z \sim q_\eta(z)} \left[ f_\eta(z) \right] = \sum_{k = 1}^K q_\eta(z = k) f_\eta(k),
\label{eq:objective_fun}
\end{align}
where the real-valued integrand $f_\eta$ also depends differentiably on $\eta$. If $K$ is finite and small enough, we can compute the exact gradient as 
\begin{align}
\begin{split}
\nabla_\eta &\E_{q_\eta(z)}[f_\eta(z)]\\
&=  \sum_{z = 1}^K \Big\{\left[\nabla_\eta q_\eta(z) \right] f_\eta(z) 
+ q_\eta(z)\nabla_\eta f_\eta(z) \Big\},
\label{eq:analytic_gradient}
\end{split}
\end{align}
provided $f_\eta$ is sufficiently regular to permit differentiation under the integral (which we assume throughout). On the other hand, $K$ may be infinite, or large relative to the cost of evaluating $q_\eta \cdot f_\eta$. In either of these cases, which are the focus of this paper, the exact gradient is computationally intractable. Thus, in order to optimize $\mathcal L(\eta)$, we seek low-variance stochastic approximations of the gradient. 

The recently popularized reparametrization trick~\cite{kingma2014auto} provides efficient stochastic gradients when $q_\eta$ is a continuous distribution,
but it does not apply in the setting of discrete $z$. 
Two well-known possibilities in the discrete case are continuous relaxation~\cite{maddison2017concrete,jang2017categorical} and REINFORCE~\cite{williams1992simple} (also known as the score function estimator). The former often requires $O(K)$ computation, making it unsuitable for the setting of this paper, and is biased. The latter is known for its high variance.

Control variates are a popular mechanism for reducing the variance of REINFORCE. REBAR~\cite{tucker2017rebar} and RELAX~\cite{grathwohl2018backpropagation}, however, combine continuous relaxations with control variates, so they too
require $O(K)$ computation and are infeasible in our setting.
Other approaches use control variates that can be computed in constant time~\cite{mnih2014neural,mnih2016variational},
but these do not reduce the variance enough for many applications.

We propose here a meta-procedure that can be applied to any discrete-distribution stochastic-gradient procedure (e.g., REINFORCE, REINFORCE with control variate) to reduce its variance without changing its bias. In particular, an unbiased stochastic gradient remains unbiased after application of our technique. Further, our method is ``anytime'' in the sense that it can reduce stochastic-gradient variances given any computational budget, and the larger the budget, the greater the variance reduction. Hence it is well suited to our chosen setting, where $K$ is infinite or very large, and/or $q_\eta \cdot f_\eta$ is expensive to evaluate.

We show that our variance-reduction meta-procedure is an instance of a general statistical method called Rao-Blackwellization~\cite{casella1996rao}. Rao-Blackwellization has been used in previous work \cite{bbVI, TitsiasLocalExpGrads}, but in a setting to reduce the variance of multivariate random variables by taking advantage their conditional dependencies. We focus here on a single discrete random variable with many categories. 

The rest of the paper is organized as follows. Section 2 presents our variance-reduction meta-procedure. Section 3 makes the connection to Rao-Blackwellization, proves that the technique necessarily reduces stochastic-gradient variances, and proves that any computational budget is better spent on our technique than on simple stochastic-gradient minibatching. In Section 4, we exhibit the benefits of our procedure on synthetic data as well as on an attention mechanism~\cite{mnihattnmechanism, GregorDRAW} for galaxy detection in astronomical images. Section 5 closes.


% \todo[inline]{It may be more about avoiding $\mathcal O(K^2)$ actually. Because $q(z)$ is length $K$ vector. But we don't want to have to run the decoder once for each of the $K$ pixels, since each run of the decoder generates a $2K$ dimensional output.}

% \todo[inline]{In our experiments, we use a different control variates for REINFORCE and for our procedure. 
% They're related, but not exactly the same.
% Not sure how to handle that.}

% \subsection{Method}

% \todo[inline]{Let's incorporate the parts of this subsection that we keep into the introduction above.}
% \todo[inline]{We also need to include a discussion explaining why evaluating $q_{\eta}(z)$ is cheap but evaluating $f(z)$ is expensive in variational inference; I'm not sure if this tied to hard attention/VAE style problem.}
% If $z$ takes on only a few discrete categories, say $z \in \{1, ..., K\}$, then this expectation can be evaluated analytically: 
% \begin{align}
% \E_{q_\eta(z)}[f(z)] = \sum_{k = 1}^K q_\eta(z = k) f_\eta(k)
% \label{eq:analytic_expectation}
% \end{align}
% If this sum can be evaluated, then we do not require stochastic gradients, and can compute
% \begin{align}
% \nabla_\eta &\E_{q_\eta(z)}[f_\eta(z)] = \notag \\  &\sum_{k = 1}^K \Big\{\nabla_\eta q_\eta(z = k) f_\eta(k) 
% + q_\eta(z = k)\nabla_\eta f_\eta(k) \Big\}
% \end{align}

% However, in many applications the $K$ is large so this sum is intractable. Moreover, querying the function $f$ $K$ times may be expensive. A sigmoid belief network CITE illustrates both of these challenges, as the evaluation of $f$ requires a forward pass through a neural network, and if there are $d$ Bernoulli latent parameters, then there are $2^d$ categories to sum. 

% To compute gradients then, several estimators have been proposed. For example, one may compute $\nabla \mathcal{L}(\eta)$ as 
% \begin{align}
%     \nabla_\eta \mathcal{L}(\eta) = \E_{q_\eta(z)}[f_\eta(z) \nabla_\eta \log q_\eta(z) + \nabla_\eta f_\eta(z)]
%     \label{eq:reinforce_estimate}
% \end{align}
% which we estimate with a draw $z \sim q_\eta(z)$ and evaluate $f_\eta(z) \nabla_\eta q_\eta(z) + \nabla_\eta f_\eta(z) $. This is known as the REINFORCE estimator CITE and is an unbiased estimate of the true gradient. However, this estimator is generally too high variance to be of use in practice. Others have suggested the use of control variates to address this issue. For a control variate, the key observation is that the score function $\nabla_\eta q_\eta(z)$ has expectation 0 under $q_\eta(z)$, and therefore, an estimator of the form 
% \begin{align}
%     [f_\eta(z) - C]\nabla_\eta \log q_\eta(z)  + \nabla_\eta f_\eta(z) \quad z \sim q_\eta(z)
%     \label{eq:reinforce_w_control_estimate}
% \end{align}
% is still unbiased for the true gradient. Several proposals have been put forth and are used in practice to choose values of $C$ to then reduce the variance of the estimator CITE. 

% Others have proposed a continuous relaxation to the discrete random variable, and therefore they can apply the reparameterization trick CITE. While these methods reduce variance, the estimator is no longer unbiased. 

% A recent method includes the ARM gradient estimator CITE, which combines both a continuous relaxation of the discrete random variable and the REINFORCE estimator to obtain low variance, unbiased estimates of the gradient. 

% In this paper, we present a \textit{meta-procedure} that can be applied on top of any of the existing methods. We propose to decompose the expectation in \ref{eq:analytic_expectation} into two components: a portion where $q$ is \textit{concentrated}, and a portion where $q$ is \textit{diffuse}. We then compute deterministic gradients for the concentrated portion, and use any stochastic estimator for the diffuse portion. The inspiration comes from observing that in many applications, $q_\eta(z)$ only puts significant mass on a few categories; by integrating out these areas where $q_\eta(z)$ is concentrated, we are nearly recovering the exact expectation, and hence our deterministic gradient is nearly correct. A small stochastic estimator is added, to correct for the remaining error. 


% Formally, let $G(z)$ be any estimator which satisfies $\E_{z}[G(z)] = \nabla_{\eta} \E_{q_{\eta}(z)} [f(z)]$
% (e.g. the REINFORCE estimator). Let $\mathcal{C}_\alpha = \{z : q_\eta(z) > \alpha\}$, the set where $q_\eta(z)$ has mass greater than some value $\alpha$. 
% We write
% \begin{align}
%  \E_{q_\eta(z)}[G(z)] &=
%  \E_{q_\eta(z)}[G(z) \Ind\{z \in \mathcal{C}_\alpha\} + G(z) \Ind\{z \not\in \mathcal{C}_\alpha\}] \\
% &= \sum_{z\in\mathcal{C}_\alpha}q_\eta(z) G(z) + \E_{q_\eta(z)}[G(z)\Ind\{z \not\in \mathcal{C}_\alpha\}]
% \label{eq:partial_marg_decomp}
% \end{align}
% It remains to approximate the expectation of the second term. Naively, if we sample $z\sim q_\eta(z)$ and compute $G(z)\Ind\{z \not\in \mathcal{C}_\alpha\}$, it is unlikely that the variance of this estimator improves on the original estimate. This is because $G(z)\Ind\{z \not\in \mathcal{C}_\alpha\}$ is by definition zero where $q_\eta$ has large mass, and non-zero where $q_\eta$ has small mass. 

% This situation then suggests that we estimate the expectation using importance sampling. A particularly simple choice of an importance distribution is the conditional distribution of $q_\eta$ restricted to the complement of $C_\alpha$. That is, we sample $z \sim q_\eta(z | z\not\in C_\alpha)$, compute $G(z)$, and renormalize by $q_\eta(z\not\in C_\alpha)$ (note that the indicator then is always 1 because we are only sampling from $z\not\in C_\alpha$. 

% In sum, we estimate the gradient as
% \begin{align}
%     & P(z') = \sum_{z \in C_{\alpha}} q_{\eta}(z) G(z) + q_{\eta}(z \notin C_{\alpha}) G(z') \label{eq:pm_estimate} \\
%     & \quad z' \sim q_{\eta}(z' | z' \notin \mathcal{C}_{\alpha}) \notag
% \end{align}
% We call this the partially marginalized (over the set $\mathcal{C}_{\alpha}$) estimator, and it also satisfies $\E_{z'}[P(z')] = \nabla_{\eta} \E_{q_{\eta}(z)} [f(z)]$.

% We see that the first term of this estimator is deterministic; and the second term is random, but scaled by $q_\eta(z\notin C_\alpha)$, which is chosen to be small. Therefore, we expect this estimator to have smaller variance than the original estimator, $G(z)$. 

% Alternatively, if $g(z), z\sim q_\eta(z)$ is unbiased for the true gradient, (e.g. $g(z)$ is the REINFORCE estimator), then we can do 
% \begin{align}
%     \nabla_\eta \E_{q_\eta(z)}[f(z)] &= \E_{q_\eta(z)}[g(z)]\\ 
%     &= \sum_{z\in\mathcal{C}_\alpha}q_\eta(z) g(z) + \\ &q_\eta(z\not\in \mathcal{C}_\alpha)\cdot \E_{q_\eta(z)}[g(z) | z \not\in \mathcal{C}_\alpha]
% \end{align}
% So we get an unbiased estimate for the gradient by computing 
% \begin{align}
% \sum_{z\in\mathcal{C}_\alpha}q_\eta(z) g(z) + q_\eta(z\not\in \mathcal{C}_\alpha)g(z') 
% \end{align}
% where $z'$ is one draw from the conditional distribution $q_\eta(z | z \not\in \mathcal{C}_\alpha)$. 


% ------------ idea 3 ------------ 

% More formally, let $\mathcal{C}_\alpha = \{z : q_\eta(z) > \alpha\}$, the set where $q_\eta(z)$ has mass greater than some value $\alpha$, and $\Ind \{z\in \mathcal{C}_\alpha\}$ be the indicator that $z\in\mathcal{C}_\alpha$. We write
% \begin{align}
%  \E_{q_\eta(z)}[f(z)] &=
%  \E_{q_\eta(z)}[f(z) \Ind\{z \in \mathcal{C}_\alpha\} + f(z) \Ind\{z \not\in \mathcal{C}_\alpha\}] \\
% &= \sum_{z\in\mathcal{C}_\alpha}q_\eta(z) f(z) + \E_{q_\eta(z)}[f(z)\Ind\{z \not\in \mathcal{C}_\alpha\}]
% \end{align}

% We take a gradient of this objective, and use any stochastic gradient estimator for the second term. For example, if we use REINFORCE for the second term, then we draw $z \sim q_\eta(z)$ and 
% \begin{align}
%     \sum_{z'\in\mathcal{C}_\alpha}\nabla_\eta q_\eta(z') f(z') + f(z)\Ind\{z \not\in \mathcal{C}_\alpha\}\nabla_\eta\log q_\eta(z)
% \end{align}
% is an unbiased estimator for the gradient. 

% Hence, to a deterministic gradient, we an occasional stochastic correction to ensure it is unbiased. 

